HorizANN: Elastically Scaling Vector Search with Ghost Edges

Approximate nearest neighbor search (ANNS) is fundamental to modern data-intensive AI applications such as retrieval-augmented generation, recommendation systems, and semantic search. Among existing indexing methods, graph-based indexes emerge as the state of the art due to their superior recall-throughput tradeoffs. Scaling these indexes to multiple machines requires partitioning the data and building indexes on each. However, when new machines are added or removed, the data must be repartitioned and the indexes reconstructed from scratch, making horizontal scaling costly at billion scale. In this work, we present HorizANN, a distributed graph-based ANNS system that scales horizontally without requiring full index reconstruction. To achieve this, we introduce ghost edges, a mechanism for preserving cross-partition connectivity as partition boundaries change during repartitioning. By reusing the structural information that would otherwise be discarded during repartitioning, HorizANN avoids costly full index reconstruction. As the index grows from 100M vectors on one worker to 1B vectors on ten workers, HorizANN inserts each 100M vectors within 2.5 hours and sustains 3.4--3.5K queries per second at 0.998 Recall@10.

==> figures/1_intro/rebalancing-break_v0.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}[
        scale=1.0,
        every node/.style={transform shape},
        vnode/.style={circle, draw=cZmain!80, fill=white, line width=0.8pt, minimum size=5.2mm, inner sep=0pt},
        box2/.style={draw=cBmain, line width=1.0pt, rounded corners=2.5pt},
        box3/.style={draw=cAmain, line width=1.0pt, rounded corners=2.5pt},
        intra_edge/.style={draw=cZmain!75, line width=0.9pt},
        new_intra/.style={draw=cAmain, line width=1.1pt},
        severed_edge/.style={draw=cBmain, line width=1.5pt, dashed},
        boxlabel2/.style={font=\small\bfseries, text=cBmain},
        boxlabel3/.style={font=\small\bfseries, text=cAmain},
        lostlabel2/.style={font=\footnotesize, text=cBmain}
    ]

    % Nodes
    \node[vnode] (v1) at (0.5, 0.5) {};
    \node[vnode] (v2) at (1.3, 1.1) {};

    \node[vnode] (v3) at (2.4, 1.7) {};
    \node[vnode] (v4) at (2.4, 0.4) {};
    \node[vnode] (v5) at (3.6, 1.0) {};

    \node[vnode] (v6) at (4.7, 1.55) {};
    \node[vnode] (v7) at (4.8, 0.45) {};

    % Intra-partition edges (standard)
    \draw[intra_edge] (v1) -- (v2);
    \draw[intra_edge] (v3) -- (v4);
    \draw[intra_edge] (v6) -- (v7);

    % New intra-partition edges (between v3, v4, v5 in w2/3)
    \draw[new_intra] (v3) -- (v5);
    \draw[new_intra] (v4) -- (v5);

    % Severed cross-boundary edges (were in 2-worker partitions, now severed by 3-worker split)
    \draw[severed_edge] (v2) -- node[above, sloped, lostlabel2] {lost} (v3);
    \draw[severed_edge] (v2) -- node[above, sloped, lostlabel2] {lost} (v4);
    \draw[severed_edge] (v5) -- node[above, sloped, lostlabel2] {lost} (v6);
    \draw[severed_edge] (v5) -- node[above, sloped, lostlabel2] {lost} (v7);

    % 2-Worker BBoxes (top label)
    \draw[box2] (0.05, -0.05) rectangle (2.85, 2.3);
    \node[boxlabel2] at (1.45, 2.5) {$w_{1/2}$};

    \draw[box2] (3.15, -0.05) rectangle (5.25, 2.3);
    \node[boxlabel2] at (4.2, 2.5) {$w_{2/2}$};

    % 3-Worker BBoxes (bottom label)
    \draw[box3] (-0.05, -0.2) rectangle (1.75, 2.1);
    \node[boxlabel3] at (0.85, -0.42) {$w_{1/3}$};

    \draw[box3] (1.95, -0.2) rectangle (4.05, 2.1);
    \node[boxlabel3] at (3.0, -0.42) {$w_{2/3}$};

    \draw[box3] (4.25, -0.2) rectangle (5.35, 2.1);
    \node[boxlabel3] at (4.8, -0.42) {$w_{3/3}$};
    \end{tikzpicture}
    % \includegraphics[width=0.7\linewidth]{figures/1_intro/rebalancing-break-draft.png}
    \caption{Naive cluster re-balancing severs cross-partition edges. When data vectors migrate from 2 workers (\textbf{\color{cBmain}{orange}}) to 3 workers (\textbf{\color{cAmain}{blue}}), edges intersecting the new partition boundaries are permanently lost (\textbf{\color{cBmain}{orange edges}}), rendering the local graphs mutually unreachable during greedy routing. {\color{red} Show the before \& after difference. We firstly talk about how to search on multiple nodes with bulk build (ideal), and show something bad happens when there is no ghost edges. We just want to show even if we can not be the same as ideal case, without ghost edges the scenario will be worse. We want to show the KNN property, which means a node should connect to its nearest neighbors, but in our scenario, we can maintain the property by ghost edges while without ghost edges we may lose it. And we need to save the graph index, to avoid the reviewers challenge we don't measure the KNN property, so we can directly calculate it.}}
    \label{fig:rebalancing-break}
\end{figure}

==> figures/2_method/merge_figure.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[
    scale=1.1,
    transform shape,
    vertex/.style={circle, draw=cZmain, minimum size=5mm, inner sep=0pt, font=\scriptsize},
    vertex_a/.style={vertex, fill=cAlight, draw=cAmain},
    vertex_b/.style={vertex, fill=cBlight, draw=cBmain},
    active_edge/.style={-, semithick, draw=cZmain!85},
    ghost_edge/.style={-, dashed, semithick, draw=cZmain!40},
    reactivated_edge/.style={-, semithick, draw=cCmain},
    arrow/.style={->, thick, >=stealth, draw=cZmain},
    label_style/.style={font=\scriptsize},
    box/.style={draw=cZmain!60, rounded corners, inner sep=3pt}
]

% === Before Merge ===
\node[label_style] at (0.9, 2.2) {\textbf{Before Merge}};

% Partition P_a
\node[vertex_a] (a1) at (-0.4, 1.3) {$v_1$};
\node[vertex_a] (a2) at (-0.6, 0.6) {$v_2$};
\node[vertex_a] (a3) at (0.0, 0.1) {$v_3$};
\node[vertex_a] (a4) at (0.3, 0.8) {$v_4$};

\draw[active_edge] (a1) -- (a2);
\draw[active_edge] (a2) -- (a3);
\draw[active_edge] (a3) -- (a4);
\draw[active_edge] (a4) -- (a1);
\draw[active_edge] (a1) -- (a3);

\node[box, fit=(a1)(a2)(a3)(a4), label={[label_style]above:$P_a$}] {};

% Partition P_b
\node[vertex_b] (b1) at (2.0, 1.2) {$v_5$};
\node[vertex_b] (b2) at (2.4, 0.5) {$v_6$};
\node[vertex_b] (b3) at (1.9, -0.1) {$v_7$};

\draw[active_edge] (b1) -- (b2);
\draw[active_edge] (b2) -- (b3);
\draw[active_edge] (b1) -- (b3);

\node[box, fit=(b1)(b2)(b3), label={[label_style]above:$P_b$}] {};

% Ghost edges between partitions
\draw[ghost_edge] (a1) -- (b1);
\draw[ghost_edge] (a4) -- (b1);
\draw[ghost_edge] (a3) -- (b3);
\draw[ghost_edge] (a4) -- (b2);

% === ARROW ===
\draw[arrow] (2.9, 0.6) -- (3.5, 0.6);
\node[font=\scriptsize] at (3.2, 0.85) {Merge};

% === RIGHT: After Merge ===
\node[label_style] at (5.2, 2.2) {\textbf{After Merge}};

% Merged partition
\node[vertex_a] (a1r) at (4.2, 1.3) {$v_1$};
\node[vertex_a] (a2r) at (4.0, 0.6) {$v_2$};
\node[vertex_a] (a3r) at (4.6, 0.1) {$v_3$};
\node[vertex_a] (a4r) at (4.9, 0.8) {$v_4$};

\node[vertex_b] (b1r) at (5.9, 1.2) {$v_5$};
\node[vertex_b] (b2r) at (6.3, 0.5) {$v_6$};
\node[vertex_b] (b3r) at (5.8, -0.1) {$v_7$};

% Original P_a edges
\draw[active_edge] (a1r) -- (a2r);
\draw[active_edge] (a2r) -- (a3r);
\draw[active_edge] (a3r) -- (a4r);
\draw[active_edge] (a4r) -- (a1r);
\draw[active_edge] (a1r) -- (a3r);

% Original P_b edges
\draw[active_edge] (b1r) -- (b2r);
\draw[active_edge] (b2r) -- (b3r);
\draw[active_edge] (b1r) -- (b3r);

% Reactivated ghost edges (now active)
\draw[active_edge] (a1r) -- (b1r);
\draw[active_edge] (a4r) -- (b1r);
\draw[active_edge] (a3r) -- (b3r);
\draw[active_edge] (a4r) -- (b2r);

\node[box, fit=(a1r)(a2r)(a3r)(a4r)(b1r)(b2r)(b3r), label={[label_style]above:$P$}] {};

% === LEGEND ===
\node[label_style] at (3.0, -0.9) {
    \tikz[baseline=-0.5ex]{\draw[active_edge] (0,0) -- (0.3,0);} Active \;
    \tikz[baseline=-0.5ex]{\draw[ghost_edge] (0,0) -- (0.3,0);} Ghost \;
    % \tikz[baseline=-0.5ex]{\draw[reactivated_edge] (0,0) -- (0.3,0);} Reactivated
};

\end{tikzpicture}
\caption{Merge operation: ghost edges are reactivated to restore connectivity between $P_a$ and $P_b$.}
\label{fig:merging_figure}
\end{figure}

==> figures/2_method/rebalancing_flow_diagram.tex <==

\begin{figure*}[t]
    \centering
\begin{tikzpicture}[
    worker/.style={draw=cAmain, rounded corners=3pt, minimum height=1cm, 
                   minimum width=1.2cm, align=center, font=\scriptsize,
                   fill=white},
    worker_new/.style={draw=cCmain, rounded corners=3pt, minimum height=1cm, 
                   minimum width=1.2cm, align=center, font=\scriptsize,
                   fill=cClight, dashed},
    worker_overload/.style={draw=cDmain, rounded corners=3pt, minimum height=1cm, 
                   minimum width=1.2cm, align=center, font=\scriptsize,
                   fill=cDlight},
    child_index/.style={draw=cBmain, rounded corners=1pt, minimum height=0.4cm, 
                  minimum width=0.45cm, align=center, font=\tiny,
                  fill=cBlight},
    step/.style={circle, draw=cZmain, fill=white, font=\scriptsize\bfseries, 
                 inner sep=1pt, minimum size=14pt},
    arrow/.style={-{Stealth[scale=0.7]}, very thick, cAmain!60},
    transfer/.style={-{Stealth[scale=0.5]}, densely dashed, cBmain, thick},
    phase/.style={font=\small\bfseries},
    desc/.style={font=\scriptsize, align=center}
]

% ============================================
% PHASE 1: Initial State
% ============================================
\node[worker] (w1a) at (0, 0) {$W_1$};
\node[worker_overload] (w2a) at (1.4, 0) {$W_2$};

\node[phase] at (0.7, 1.3) {Initial Cluster};
\node[step=1cm] at (0.7, -1) {1};
\node[desc] at (0.7, -1.55) {Provision $W_3$};

% ============================================
% Arrow to phase 2
% ============================================
\draw[arrow] (2.3, 0) -- (3.2, 0);

% ============================================
% PHASE 2: Repartition
% ============================================
\node[worker, minimum width=0.9cm] (w1b) at (3.8, 0) {$W_1$};
\node[worker, minimum width=0.9cm] (w2b) at (4.8, 0) {$W_2$};
\node[worker_new, minimum width=0.9cm] (w3b) at (5.8, 0) {$W_3$};

\node[phase] at (4.8, 1.3) {Reclustering};
\node[step=1cm] at (4.8, -1) {2};
\node[desc] at (4.8, -1.55) {Balanced $k$-means, update $\pi$};

% ============================================
% Arrow to phase 3
% ============================================
\draw[arrow] (6.5, 0) -- (7.4, 0);

% ============================================
% PHASE 3: Local Split
% ============================================
% W1 splits into I1, I2
\node[worker, minimum width=1.5cm, minimum height=1.2cm] (w1c) at (8.2, 0) {};
\node[font=\scriptsize\bfseries] at (8.2, 0.35) {$W_1$};
\node[child_index] (w1c1) at (7.95, -0.15) {$I_1$};
\node[child_index] (w1c2) at (8.45, -0.15) {$I_2$};

% W2 splits into I1, I2, I3
\node[worker, minimum width=1.9cm, minimum height=1.2cm] (w2c) at (10.1, 0) {};
\node[font=\scriptsize\bfseries] at (10.1, 0.35) {$W_2$};
\node[child_index] (w2c1) at (9.65, -0.15) {$I_1$};
\node[child_index] (w2c2) at (10.1, -0.15) {$I_2$};
\node[child_index] (w2c3) at (10.55, -0.15) {$I_3$};

\node[phase] at (9.2, 1.3) {Split};
\node[step=1cm] at (9.2, -1) {3};
\node[desc] at (9.2, -1.55) {Local split by $\pi$};

% ============================================
% Arrow to phase 4
% ============================================
\draw[arrow] (11.3, 0) -- (12.2, 0);

% ============================================
% PHASE 4: Transfer & Merge
% ============================================
% Final W1 receives I1 from W1 and W2
\node[worker, minimum width=1.5cm, minimum height=1.2cm] (w1d) at (13, 0) {};
\node[font=\scriptsize\bfseries] at (13, 0.35) {$W_1$};
\node[child_index] (w1d1) at (12.75, -0.15) {$I_1$};
\node[child_index] (w1d2) at (13.25, -0.15) {$I_1$};

% Final W2 receives I2 from W1 and W2
\node[worker, minimum width=1.5cm, minimum height=1.2cm] (w2d) at (14.6, 0) {};
\node[font=\scriptsize\bfseries] at (14.6, 0.35) {$W_2$};
\node[child_index] (w2d1) at (14.35, -0.15) {$I_2$};
\node[child_index] (w2d2) at (14.85, -0.15) {$I_2$};

% Final W3 receives I3 from W2
\node[worker, minimum width=1.2cm, minimum height=1.2cm] (w3d) at (16, 0) {};
\node[font=\scriptsize\bfseries] at (16, 0.35) {$W_3$};
\node[child_index] (w3d1) at (16, -0.15) {$I_3$};

\node[phase] at (14.5, 1.3) {Merge};
\node[step=1cm] at (14.5, -1) {4};
\node[desc] at (14.5, -1.55) {Merge via ghost edges};

% Transfer arrows with label
\draw[transfer, bend left=35] (w1c2.north) to (w2d1.north);
\draw[transfer, bend left=35] (w2c1.north) to (w1d2.north);
\draw[transfer, bend left=45] (w2c3.north) to (w3d1.north);

% Transfer label above arrows
\node[font=\scriptsize, text=cBmain] at (12, 1.5) {Transfer Indices};

\end{tikzpicture}
    \caption{Rebalancing protocol. When $W_2$ exceeds capacity, a new worker $W_3$ is provisioned. Balanced $k$-means recomputes partition assignments $\pi$, each worker splits its local index, and child indices are transferred to their assigned destinations. Receiving workers merge indices using ghost edge reactivation.}
    \label{fig:rebalancing}
\end{figure*}




==> figures/2_method/split_figure.tex <==

\begin{figure}[t]
\centering
\begin{tikzpicture}[
    scale=1.1,
    transform shape,
    vertex/.style={circle, draw=cZmain, minimum size=5mm, inner sep=0pt, font=\scriptsize},
    vertex_a/.style={vertex, fill=cAlight, draw=cAmain},
    vertex_b/.style={vertex, fill=cBlight, draw=cBmain},
    active_edge/.style={-, semithick, draw=cZmain!85},
    ghost_edge/.style={-, dashed, semithick, draw=cZmain!40},
    cross_edge/.style={-, semithick, draw=cDmain},
    arrow/.style={->, thick, >=stealth, draw=cZmain},
    label_style/.style={font=\scriptsize},
    box/.style={draw=cZmain!60, rounded corners, inner sep=3pt}
]

% === Before Split ===
\node[label_style] at (0, 1.9) {\textbf{Before Split}};

% P_a vertices 
\node[vertex_a] (a1) at (-0.9, 1.3) {$v_1$};
\node[vertex_a] (a2) at (-1.1, 0.6) {$v_2$};
\node[vertex_a] (a3) at (-0.5, 0.1) {$v_3$};
\node[vertex_a] (a4) at (-0.2, 0.8) {$v_4$};

% P_b vertices
\node[vertex_b] (b1) at (0.6, 1.2) {$v_5$};
\node[vertex_b] (b2) at (1.0, 0.5) {$v_6$};
\node[vertex_b] (b3) at (0.5, -0.1) {$v_7$};

% Intra P_a edges
\draw[active_edge] (a1) -- (a2);
\draw[active_edge] (a2) -- (a3);
\draw[active_edge] (a3) -- (a4);
\draw[active_edge] (a4) -- (a1);
\draw[active_edge] (a1) -- (a3);

% Intra P_b edges
\draw[active_edge] (b1) -- (b2);
\draw[active_edge] (b2) -- (b3);
\draw[active_edge] (b1) -- (b3);

% Cross-partition edges
\draw[cross_edge] (a1) -- (b1);
\draw[cross_edge] (a4) -- (b1);
\draw[cross_edge] (a3) -- (b3);
\draw[cross_edge] (a4) -- (b2);

% === ARROW ===
\draw[arrow] (1.4, 0.6) -- (2.0, 0.6);
\node[label_style] at (1.65, 0.85) {Split};

% \node[box, fit=(a1)(a2)(a3)(a4)(b1)(b2)(b3),
%       inner sep=6pt,
%       label={[label_style]above:$P$}] {};

% After Split 
\node[label_style] at (4.5, 1.9) {\textbf{After Split}};

% Partition P_a
\node[vertex_a] (a1r) at (2.7, 1.3) {$v_1$};
\node[vertex_a] (a2r) at (2.5, 0.6) {$v_2$};
\node[vertex_a] (a3r) at (3.1, 0.1) {$v_3$};
\node[vertex_a] (a4r) at (3.4, 0.8) {$v_4$};

\draw[active_edge] (a1r) -- (a2r);
\draw[active_edge] (a2r) -- (a3r);
\draw[active_edge] (a3r) -- (a4r);
\draw[active_edge] (a4r) -- (a1r);
\draw[active_edge] (a1r) -- (a3r);

\node[box, fit=(a1r)(a2r)(a3r)(a4r), label={[label_style]above:$P_a$}] {};

% Partition P_b
\node[vertex_b] (b1r) at (5.4, 1.2) {$v_5$};
\node[vertex_b] (b2r) at (5.8, 0.5) {$v_6$};
\node[vertex_b] (b3r) at (5.3, -0.1) {$v_7$};

\draw[active_edge] (b1r) -- (b2r);
\draw[active_edge] (b2r) -- (b3r);
\draw[active_edge] (b1r) -- (b3r);

\node[box, fit=(b1r)(b2r)(b3r), label={[label_style]above:$P_b$}] {};

% Ghost edges
\draw[ghost_edge] (a1r) -- (b1r);
\draw[ghost_edge] (a4r) -- (b1r);
\draw[ghost_edge] (a3r) -- (b3r);
\draw[ghost_edge] (a4r) -- (b2r);

% === LEGEND ===
\node[label_style] at (2.3, -0.7) {
    \tikz[baseline=-0.5ex]{\draw[active_edge] (0,0) -- (0.3,0);} Active \;
    \tikz[baseline=-0.5ex]{\draw[ghost_edge] (0,0) -- (0.3,0);} Ghost \;
    \tikz[baseline=-0.5ex]{\draw[cross_edge] (0,0) -- (0.3,0);} Cross-partition
};

\end{tikzpicture}
\caption{Split operation: cross-partition edges (red) become ghost edges (dashed). This operation is repeated at each level of the HNSW index.}
\label{fig:splitting_figure}
\end{figure}




